Embedding bounded degree spanning trees in random graphs

We prove that if a tree $T$ has $n$ vertices and maximum degree at most $\Delta$, then a copy of $T$ can almost surely be found in the random graph $\mathcal{G}(n,\Delta\log^5 n/n)$.

==> 6proofthm.tex <==

\subsection{Finding flexible paths}


\pr 

\oof








